Once upon a time step: A closed-loop approach to robust MPC design

A novel perspective on the design of robust model predictive control (MPC) methods is presented, whereby closed-loop constraint satisfaction is ensured using recursive feasibility of the MPC optimization. Necessary and sufficient conditions are derived for recursive feasibility, based on the effects of model perturbations and disturbances occurring at one time step. Using these conditions and Farkas' lemma, sufficient conditions suitable for design are formulated. The proposed method is called a closed-loop design, as only the existence of feasible inputs at the next time step is enforced by design. This is in contrast to most existing formulations, which compute control policies that are feasible under the worst-case realizations of all model perturbations and exogenous disturbances in the MPC prediction horizon. The proposed method has an online computational complexity similar to nominal MPC methods while preserving guarantees of constraint satisfaction, recursive feasibility and stability. Numerical simulations demonstrate the efficacy of our proposed approach.

==> extras.tex <==

% \section{Extensions}
% The central idea of this work is that recursive feasibility implies constraint satisfaction, as discussed in Proposition \ref{Prop:RF_RCS}. This idea was then used to compute the different components of the robust MPC controller in Sections \ref{Sec:SuffCond_Feedback} and \ref{Sec:AlgProp}.  

% In this section, two extensions which use Proposition \ref{Prop:RF_RCS} are highlighted. First, it is shown that the proposed method can recover recursive feasibility in the traditional sense, i.e., with a back-up controller which does not require optimization.
% Second, it is shown that as a result of Proposition \ref{Prop:RF_RCS}, the design of robustness in MPC controllers can be completely decoupled from the performance objectives and the prediction horizon. 

% \subsection{Additive disturbances}
% In this section, consider the situation that $B_p=0$, i.e, the dynamics \eqref{eq:Dynamics1} are not affected by the perturbation term $p_k$. Such an uncertainty structure has been well-studied in literature \cite{zanon2021similarity,alvarado2022tractable}, and constraint tightening is one of the most popular design strategy for robust MPC in this problem setting \cite{chisci2001systems,parsi2022computationally}. 

% The closed loop approach for robust MPC can be simplified in this setting, as $\Delta_k$ does not affect the system dynamics. Moreover, existing constraint tightening methods such as \cite{parsi2022computationally} always provide a feasible initial guess of $\mathbf{t}$ to solve \eqref{eq:OfflineOpt}. 

% As the design is independent of the vertices $\Delta^j$, the superscript $^j$ can be removed from the design criteria formulated in Sections \ref{Sec:RCS_RF} and \ref{Sec:SuffCond_Feedback}. Moreover, the feedback structure used for design is of the form 
% \begin{align}\label{eq:InputParameterization_dist}
%     \hat{u}_{i|k+1} &= \hat{u}_{i+1|k} + M_i B_w w_k , \: \forall i \in \mathbb{N}_{0}^{N-2} \nonumber\\
%     \hat{u}_{N-1|k+1}&= K \hat{x}_{N|k} + M_{N{-}1} B_w w_k,
% \end{align}
% which is based on the disturbance feedback parameterization proposed in \cite{goulart2006optimization} and used in \cite{parsi2022computationally}. Using the feedback \eqref{eq:InputParameterization_dist}, the offline optimization \eqref{eq:OfflineOpt} can be modified as
% \begin{subequations}\label{eq:OfflineOpt_dist}
% \begin{align}
%     \min_{\substack{\mathbf{t},  K, \alpha,  \\
%   \{\mathbf{u}^{i}\}_{i=1}^{2n_x}, \Lambda,  \mathbf{M}}} &\norm{\mathbf{t}}_2 - \mu \alpha \label{eq:OfflineOpt_dist1}\\
%     \text{s.t.} \qquad &     \Lambda \ge 0, \quad \alpha > 0, \quad t_0 > 0, \label{eq:OfflineOpt_dist2}\\
%         \Lambda \begin{bmatrix}
%         \mathbf{H}_{xu}\mathbf{S} & 0 \\
%         0 & H_w
%     \end{bmatrix} &= \mathbf{H}_{xu}\begin{bmatrix}
%         \mathbf{L}_K &   \mathbf{C}_M
%     \end{bmatrix}, \label{eq:OfflineOpt_dist3}\\
%     \Lambda \begin{bmatrix}
%         \mathbf{b}-\mathbf{t} \\ h_w
%     \end{bmatrix} &\le \mathbf{b}-\mathbf{t},  \label{eq:OfflineOpt_dist4}\\
%     \mathbf{H}_{xu} \mathbf{S} \mathbf{s}^{i}_{\alpha} &\le \mathbf{b-t}, \quad \forall i \in \mathbb{N}_{1}^{2n_x}, \label{eq:OfflineOpt_dist5}
% \end{align}
% \end{subequations}
% which has fewer optimization variables and constraints compared to \eqref{eq:OfflineOpt}. Despite the reduction in problem size, \eqref{eq:OfflineOpt_dist} is also a nonconvex optimization due to the bilinear constraints \eqref{eq:OfflineOpt_dist4}. As proposed in \ref{Rem:InGuess}, an initial guess can be computed using the optimized constraint tightening (OCT) method from \cite{parsi2022computationally}. 

% \begin{Lemma}
%     Let $\mathbf{t}_\text{OCT}$ be the constraint tightenings computed using OCT. Then, $\mathbf{t}_\text{OCT}$ is a feasible set of tightenings $\mathbf{t}$ in \eqref{eq:OfflineOpt_dist}. 
% \end{Lemma}

% \subsection{Design of generic safety constraints}
% The central idea of this work is that recursive feasibility implies constraint satisfaction, as discussed in Proposition \ref{Prop:RF_RCS}. This idea was then used to design the robust MPC controller in Sections \ref{Sec:SuffCond_Feedback} and \ref{Sec:AlgProp}.  However, Proposition \ref{Prop:RF_RCS} does not restrict the robust MPC optimization to be of the structure \eqref{eq:OnlOptProb_reg}. Instead, a flexible parameterization of the following form can be used
% \begin{subequations}\label{eq:OnlOptProb_flex}
%     \begin{align}
%         \min_{\hat{\mathbf{u}}_k}  \quad  \hat{x}_{N|k}\tr &Q_N \hat{x}_{N|k} + \textstyle\sum_{i=0}^{N-1}  \hat{x}_{i|k}\tr Q_x \hat{x}_{i|k} +  \hat{u}_{i|k}\tr Q_u \hat{u}_{i|k} \label{eq:OnlOptProb_flex1} \\
% 		\text{s.t.} \quad &\hat{x}_{k,0}=x_k,\\
%             A&\hat{x}_{i|k} + B\hat{u}_{i|k} = \hat{x}_{i|k+1}, \:  \forall i\in \mathbb{N}_{0}^{N-1},\label{eq:OnlOptProb_flex2}\\
%              % &\qquad \qquad \nonumber\\
%             &F\hat{x}_{0|k} + G\hat{u}_{0|k}  \le b - t_0,   \label{eq:OnlOptProb_flex3} \\
%             &Y_f\hat{x}_{0|k} \le z_f, \label{eq:OnlOptProb_flex4}
%     \end{align}
% \end{subequations}
% where $t_0, z_f$ and $Y_f$ must be chosen by the designer. The optimization \eqref{eq:OnlOptProb_flex} is a flexible parameterization, because  \eqref{eq:OnlOptProb_reg} can be recovered for a specific choice of $Y_f$ and $z_f$. The 

%  However, the constraint \eqref{eq:OnlOptProb_flex3} needs to be explicitly imposed, as $t_0\ge0$ is explicitly used in Proposition \ref{Prop:RF_RCS}. Thus, instead of computing $\mathbf{t}$ offline using \eqref{eq:OfflineOpt}, the offline design task is to compute $t_0, Y_f$ and $z_f$.  

% \ani{
% Why impose future constraints at all? Why not just use N=1? Refute each reason for N
% \begin{itemize}
%     \item Typically, a large N can increase ROA, but here, because the terminal set can be chosen quite large, we do not need to compensate with N. 
%     \item A large N also helps to show robust constraint satisfaction explicitly. We do this implicitly using recursive feasibility, so large N is not required
% \end{itemize}
% Situations where N helps the controller:
% \begin{itemize}
%     \item N is useful when predictions of disturbances are available. For example, prices of energy, or prediction of solar radiation/changing constraints in system variables.
    
%     \item we ultimately want to approximate value function. N allows to use simple terminal costs, and still gives good value function approximations.
% \end{itemize}

% Main point: You do not need N for robust MPC (or safety) reasons. N=1 is sufficient! 
% }

